Is Your World Simulator a Good Story Presenter? A Consecutive Events-Based Benchmark for Future Long Video Generation

The current state-of-the-art video generative models can produce commercial-grade videos with highly realistic details. However, they still struggle to coherently present multiple sequential events in the stories specified by the prompts, which is foreseeable an essential capability for future long video generation scenarios. For example, top T2V generative models still fail to generate a video of the short simple story 'how to put an elephant into a refrigerator.' While existing detail-oriented benchmarks primarily focus on fine-grained metrics like aesthetic quality and spatial-temporal consistency, they fall short of evaluating models' abilities to handle event-level story presentation. To address this gap, we introduce StoryEval, a story-oriented benchmark specifically designed to assess text-to-video (T2V) models' story-completion capabilities. StoryEval features 423 prompts spanning 7 classes, each representing short stories composed of 2-4 consecutive events. We employ advanced vision-language models, such as GPT-4V and LLaVA-OV-Chat-72B, to verify the completion of each event in the generated videos, applying a unanimous voting method to enhance reliability. Our methods ensure high alignment with human evaluations, and the evaluation of 11 models reveals its challenge, with none exceeding an average story-completion rate of 50%. StoryEval provides a new benchmark for advancing T2V models and highlights the challenges and opportunities in developing next-generation solutions for coherent story-driven video generation.

==> sec/2_Relatedworks.tex <==
% \vspace{-0.5em}
\section{Related Works}
\subsection{Text-to-Video Generative Models}
% \kuan{We mainly focus on text-to-video (T2V) models}

Recent advancements in vision generation have been largely dominated by
diffusion models ~\cite{peebles2023DiT,easyanimate2024xu,opensora2024zheng,opensoraplan2024PKU_Yuan,videocrafter2_2024chen,yang2024cogvideox,vchitect2024}. The open-source release of Stable Diffusion ~\cite{rombach2022high} has catalyzed extensive research and development in this field, while closed-source models have achieved commercial-grade quality~\cite{kling2024,hailuo2024,gen3runwayml2024,pika2024}. 
In parallel, another promising research direction involves training autoregressive models for video generation, where models are trained to sequentially predict tokens for video generation ~\cite{weissenborn2019scaling_autoregressive_vg,wang2024loong_autoregressive_vg,Weng_2024_CVPR_ART_V_autoregressive_vg,moviegen2024meta,jin2024pyramid_flow,wang2024emu3, marcus2022very, ding2021cogview, yan2021videogpt, kondratyuk2023videopoet}. Despite these advancements, challenges remain in the long-term event continuity and logical narrative progression. 
Our benchmark provides a testbed for these lines of research by emphasizing the generation of coherent, long videos grounded in consecutive events. 

% Our work is designed to evaluate and drive the development of generative models capable of handling extended video sequences. By focusing on the generation of coherent long-duration content,
% such as DALL-E , CogView , Parti, VideoGPT  and VideoPoet. 

% Beyond the success of scaling video diffusion models~\cite{peebles2023DiT}, recent research has also revealed the impressive potential of autoregressive video generation. 
% This approach uses next-token prediction loss to train models, similar to language models, by tokenizing text, images, and videos into a unified discrete space~\cite{weissenborn2019scaling_autoregressive_vg,wang2024loong_autoregressive_vg,Weng_2024_CVPR_ART_V_autoregressive_vg,moviegen2024meta,jin2024pyramid_flow,wang2024emu3}.


% \subsection{Video Generation Benchmarks}
\subsection{Video Generation Metrics and Benchmarks}
The rapid advancements in text-to-video (T2V) generation have driven the development of various benchmarks to evaluate the performance of generative models across diverse dimensions~\cite{Ji_2024_T2VBench,huang2024vbench,yuan2024chronomagic_bench,feng2024TC_Bench,liu2024Fetv_Bench,meng2024PhyGenBench_world_simulator,liu2024evalcrafter_bench}. Traditional metrics like FVD \cite{unterthiner2019fvd} and IS \cite{salimans2016improved} have been widely used to assess frame quality and text-frame alignment but fall short in capturing critical aspects such as subject consistency, temporal coherence, and physical commonsense correctness, particularly for novel or dynamic scenes \cite{brooks2022generating}.
% The rapid development of text-to-video (T2V) generation models has driven the need for more advanced metrics and benchmarks to evaluate their quality across various dimensions~\cite{Ji_2024_T2VBench,huang2024vbench,yuan2024chronomagic_bench,feng2024TC_Bench,liu2024Fetv_Bench,meng2024PhyGenBench_world_simulator,liu2024evalcrafter_bench}. Traditional methods like FVD and IS focus on frame quality and video realism but struggle with capturing deeper aspects such as physical commonsense, temporal consistency, and compositional accuracy. 
Recently, benchmarks like VBench~\cite{huang2024vbench} and EvalCrafter~\cite{liu2024evalcrafter_bench} have expanded the evaluation scope, incorporating advanced metrics for dynamic attributes and human ratings. Specialized benchmarks such as T2V-CompBench~\cite{sun2024t2v} and DEVIL~\cite{liao2024evaluation}, PhyGenBench~\cite{meng2024towards} address compositional and dynamic characteristics and physical realism. However, previous methods largely focus on evaluating detailed dynamics within short videos, failing to address the broader challenge of generating coherent, story-driven long videos. To bridge this gap, our method introduces a holistic evaluation framework that emphasizes narrative completion and the accurate depiction of sequential events, providing a robust benchmark for assessing long video generative models.

% Despite these advancements, challenges remain in achieving high correlation with human ratings and effectively assessing the ability of T2V models to generate coherent, story-driven long videos. To address these challenges, our proposed method introduces a holistic evaluation framework that effectively combines fine-grained metrics, such as spatial and temporal quality, with coarse-grained metrics, like narrative completion, ensuring a robust assessment of T2V models' ability to generate coherent and story-driven long videos.

% This gap highlights the need for innovative benchmarks that holistically address both fine-grained metrics, such as spatial and temporal quality, and coarse-grained metrics, such as narrative completion, to drive future progress in the field.






% \subsection{World Model}
% \yiping{Not sure if to add this}
% \label{sec:formatting}

% All text must be in a two-column format.
% The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
% Columns are to be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
% The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
% The second and following pages should begin 1 inch (2.54 cm) from the top edge.
% On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
% for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
% page.

% %-------------------------------------------------------------------------
% \subsection{Margins and page numbering}

% All printed material, including text, illustrations, and charts, must be kept
% within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
% high.
% %
% Page numbers should be in the footer, centered and $\frac{3}{4}$ inches from the bottom of the page.
% The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
% The \LaTeX\ template takes care of this when used properly.



% %-------------------------------------------------------------------------
% \subsection{Type style and fonts}

% Wherever Times is specified, Times Roman may also be used.
% If neither is available on your word processor, please use the font closest in
% appearance to Times to which you have access.

% MAIN TITLE.
% Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
% The title should be in Times 14-point, boldface type.
% Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
% do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
% Leave two blank lines after the title.

% AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
% and printed in Times 12-point, non-boldface type.
% This information is to be followed by two blank lines.

% The ABSTRACT and MAIN TEXT are to be in a two-column format.

% MAIN TEXT.
% Type main text in 10-point Times, single-spaced.
% Do NOT use double-spacing.
% All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
% Make sure your text is fully justified---that is, flush left and flush right.
% Please do not place any additional blank lines between paragraphs.

% Figure and table captions should be 9-point Roman type as in \cref{fig:onecol,fig:short}.
% Short captions should be centred.

% \noindent Callouts should be 9-point Helvetica, non-boldface type.
% Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

% FIRST-ORDER HEADINGS.
% (For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before, and one blank line after.

% SECOND-ORDER HEADINGS.
% (For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before, and one after.
% If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period and your text on the same line.

% %-------------------------------------------------------------------------
% \subsection{Footnotes}

% Please use footnotes\footnote{This is what a footnote looks like.
% It often distracts the reader from the main flow of the argument.} sparingly.
% Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
% If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
% Use Times 8-point type, single-spaced.


% %-------------------------------------------------------------------------
% \subsection{Cross-references}

% For the benefit of author(s) and readers, please use the
% {\small\begin{verbatim}
%   \cref{...}
% \end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
% This will automatically insert the appropriate label alongside the cross-reference as in this example:
% \begin{quotation}
%   To see how our method outperforms previous work, please see \cref{fig:onecol} and \cref{tab:example}.
%   It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
%   You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
% \end{quotation}
% If you do not wish to abbreviate the label, for example at the beginning of the sentence, you can use the
% {\small\begin{verbatim}
%   \Cref{...}
% \end{verbatim}}
% command. Here is an example:
% \begin{quotation}
%   \Cref{fig:onecol} is also quite important.
% \end{quotation}

% %-------------------------------------------------------------------------
% \subsection{References}

% List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
% When referenced in the text, enclose the citation number in square brackets, for
% example~\cite{Authors14}.
% Where appropriate, include page numbers and the name(s) of editors of referenced books.
% When you cite multiple papers at once, please make sure that you cite them in numerical order like this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
% If you use the template as advised, this will be taken care of automatically.



% %-------------------------------------------------------------------------
% \subsection{Illustrations, graphs, and photographs}

% All graphics should be centered.
% In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
% Instead use
% {\small\begin{verbatim}
%   \centering
% \end{verbatim}}
% at the beginning of your figure.
% Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
% Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
% Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
% You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

% When placing figures in \LaTeX, it's almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
% {\small\begin{verbatim}
%    \usepackage{graphicx} ...
%    \includegraphics[width=0.8\linewidth]
%                    {myfile.pdf}
% \end{verbatim}
% }


% %-------------------------------------------------------------------------
% \subsection{Color}

% Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

% If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
% Hence avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.
